Order-of-Magnitude SNR Improvement for High-Field EPR Spectrometers via 3D-Printed Quasioptical Sample Holders

In this paper, we present a rapidly-prototyped, costefficient, 3D-printed quasioptical sample holder for improving the signal-to-noise ratio (SNR) in modern, resonator-free, highfield electron paramagnetic resonance (EPR) spectrometers. Such spectrometers typically operate in induction mode: the detected EPR (cross-polar) signal is polarized orthogonal to the incident (co-polar) radiation. The sample holder improves SNR in three modes: continuous wave, pulsed, and rapid-scan. An adjustable sample positioner allows for optimizing sample position to maximize the 240 GHz magnetic field B1, and a rooftop mirror allows for small rotations of the cross-polar signal to maximize the signal and minimize the co-polar background. When optimized, the co-polar isolation (the ratio of incident to detected co-polar signal) was around 50 dB, an improvement of over 20 dB. This large isolation is especially beneficial for maximizing the SNR of rapidscan EPR, but also improves the SNR in pulsed and cwEPR experiments. Through minimal modification, the sample holder may be incorporated into a variety of homebuilt, induction-mode hfEPR spectrometers in order to significantly improve the SNR (approx. 6x), and thereby reduce the acquisition time (by more than a factor of 30).

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
